Is Your LLM Secretly a World Model of the Internet? Model-Based Planning for Web Agents

Language agents based on large language models (LLMs) have demonstrated great promise in automating web-based tasks. Recent work has shown that incorporating advanced planning algorithms, e.g., tree search, is advantageous over reactive planning for web agents. However, unlike simulated sandbox environments, real-world environments such as the web are rife with irreversible actions. This undermines the feasibility of backtracking, a cornerstone of (tree) search. Overly relying on test-time search also hurts efficiency. We advocate model-based planning for web agents that employs a world model to simulate and deliberate over the outcome of each candidate action before committing to one. We systematically explore this paradigm by (1) Proposing a model-based planning framework, WebDreamer, which employs LLMs to serve as both world models and value functions; (2) Training specialized LLMs as world models with a scalable data synthesis pipeline. Empirical results demonstrate that WebDreamer achieves substantial performance improvements over reactive baselines. It is competitive, while being 4-5 times more efficient, with tree search in sandbox environments (VisualWebArena) and also works effectively on real-world websites (Online-Mind2Web and Mind2Web-Live). Furthermore, our trained world model, Dreamer-7B, performs comparable to GPT-4o, highlighting the potential of specialized world models for efficient and effective planning in complex web environments.

==> tables/main_v1.tex <==
\begin{table*}[t]
\centering
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & \textbf{Observation $\mathcal{O}$} & \textbf{Method} & \textbf{Completion Rate} & \textbf{Success Rate} \\
\midrule
\multirow{5}{*}{VisualWebArena} & \multirow{5}{*}{Screenshot+SoM}
  & \cellcolor{gray!10}Gemini-1.5-Pro + Reactive~\citep{koh2024visualwebarena}& \cellcolor{gray!10}- & \cellcolor{gray!10}12.0\%  \\
  & & \cellcolor{gray!10}GPT-4 + Reactive~\citep{koh2024visualwebarena}& \cellcolor{gray!10}- & \cellcolor{gray!10}16.4\%  \\
  \cmidrule(lr){3-5}
  & & GPT-4o + Reactive~\citep{koh2024visualwebarena} & - & \cellcolor{green!36}17.7\%$^\dagger$  \\
  & & GPT-4o + Tree Search~\citep{koh2024tree} & - & \cellcolor{green!52}26.4\% \\
  % \cmidrule(lr){3-5}
  & & GPT-4o + \OurMethod & - & \cellcolor{green!48}23.6\% (\textcolor{black}{\faArrowUp}33.3\%) \\
\midrule
\multirow{7}{*}{Mind2Web-live} & \multirow{7}{*}{HTML}
& \cellcolor{gray!10}GPT-4 + Reactive~\citep{webcanvas} & \cellcolor{gray!10}48.8\% &  \cellcolor{gray!10}23.1\%  \\
& & \cellcolor{gray!10}Claude-3-Sonnet + Reactive~\citep{webcanvas} & \cellcolor{gray!10}47.9\% &  \cellcolor{gray!10}22.1\%  \\
& & \cellcolor{gray!10}Gemini-1.5-Pro + Reactive~\citep{webcanvas} & \cellcolor{gray!10}44.6\% &  \cellcolor{gray!10}22.3\%  \\
& & \cellcolor{gray!10}GPT-4-turbo + Reactive~\citep{webcanvas} & \cellcolor{gray!10}44.3\% & \cellcolor{gray!10}21.1\%  \\
& & \cellcolor{gray!10}GPT-3.5-turbo + Reactive~\citep{webcanvas} & \cellcolor{gray!10}40.2\% & \cellcolor{gray!10}16.5\%  \\
  \cmidrule(lr){3-5}
  & & GPT-4o + Reactive~\citep{webcanvas} & 47.6\% & \cellcolor{green!42} 22.1\%  \\
  & & GPT-4o + \OurMethod  & 49.9\% & \cellcolor{green!50}25.0\% (\textcolor{black}{\faArrowUp}13.1\%)  \\
\bottomrule
\end{tabular}
}
\caption{Results on VisualWebArena and Mind2Web-live.
\OurMethod significantly outperforms the reactive baseline and falls only slightly short of the tree search baseline on VWA while requiring far fewer website interactions.
For Mind2Web-live, implementing tree search algorithms poses significant challenges due to the requirement for website backtracing, leading us to omit tree search performance metrics. 
This limitation further underscores the flexibility of our model-based planning method.
We also include additional baselines (denoted by \colorbox{gray!10}{gray} cells) to provide broader context. 
While these comparisons may not directly assess our core hypothesis, they offer valuable background for understanding our method's performance in the web navigation landscape.
$^\dagger$ We run the reactive baseline on VWA by ourselves because local hosting requirements may lead to hardware-dependent performance variations.
}
\label{tab:main}
\end{table*}

==> tables/vwa_breakdown.tex <==
\begin{table*}[h!]
\centering
\begin{minipage}{0.45\linewidth}
    \centering
    % \caption*{(a) Websites}
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Websites} & \textbf{Reactive} & \textbf{Tree Search} & \textbf{\OurMethod} &  \textbf{$\gamma$}\\
        \midrule
        Classifieds & 17.9\% & 26.8\% & 23.2\% & \cellcolor{green!50}59.6\% \\
        
        Reddit & 14.3\% & 20.6\% & 17.5\% & \cellcolor{green!30}50.8\% \\
        Shopping & 19.3\% & 28.9\% & 26.3\%  & \cellcolor{green!80}72.9\%\\
        \bottomrule
    \end{tabular}
    }
    \caption*{(a) Websites}
\end{minipage}%
\hfill
\begin{minipage}{0.45\linewidth}
    \centering
    % \caption*{(b) Task Difficulty}
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Difficulty} & \textbf{Reactive} & \textbf{Tree Search} & \textbf{\OurMethod} &  \textbf{$\gamma$}\\
        \midrule
        Easy & 28.8\% & 42.3\% & 37.4\% & \cellcolor{green!50}63.7\% \\
        Medium & 16.4\% & 22.2\% & 24.1\% & \cellcolor{green!100}132.8\%\\
        Hard & 10.7\% & 14.9\% & 12.7\% & \cellcolor{green!20}47.6\%\\
        \bottomrule
    \end{tabular}
    }
    \caption*{(b) Task Difficulty}
\end{minipage}
\caption{Success rate breakdown based on different dimensions.
$\gamma=\frac{SR_{\text{\OurMethod}}-SR_{\text{reactive}}}{SR_{\text{tree search}}-SR_{\text{reactive}}}$ measures the extent to which \OurMethod narrows the gap between the reactive agent and the tree search agent. All methods here use GPT-4o for fair comparison.}
\label{tab:fine}
\vspace{-1em}
\end{table*}
